The low-luminosity type II SN\,2016aqf: A well-monitored spectral evolution of the Ni/Fe abundance ratio

Low-luminosity type II supernovae (LL SNe~II) make up the low explosion energy end of core-collapse SNe, but their study and physical understanding remain limited. We present SN\,2016aqf, a LL SN~II with extensive spectral and photometric coverage. We measure a $V$-band peak magnitude of $-14.58$\,mag, a plateau duration of $\sim$100\,days, and an inferred $^{56}$Ni mass of $0.008 \pm 0.002$\,\msun. The peak bolometric luminosity, L$_{\rm bol} \approx 10^{41.4}$\,erg\,s$^{-1}$, and its spectral evolution is typical of other SNe in the class. Using our late-time spectra, we measure the [\ion{O}{i}] $\lambda\lambda6300, 6364$ lines, which we compare against SN II spectral synthesis models to constrain the progenitor zero-age main-sequence mass. We find this to be 12 $\pm$ 3\,\msun. Our extensive late-time spectral coverage of the [\ion{Fe}{ii}] $\lambda7155$ and [\ion{Ni}{ii}] $\lambda7378$ lines permits a measurement of the Ni/Fe abundance ratio, a parameter sensitive to the inner progenitor structure and explosion mechanism dynamics. We measure a constant abundance ratio evolution of $0.081^{+0.009}_{-0.010}$, and argue that the best epochs to measure the ratio are at $\sim$200 -- 300\,days after explosion. We place this measurement in the context of a large sample of SNe II and compare against various physical, light-curve and spectral parameters, in search of trends which might allow indirect ways of constraining this ratio. We do not find correlations predicted by theoretical models; however, this may be the result of the exact choice of parameters and explosion mechanism in the models, the simplicity of them and/or primordial contamination in the measured abundance ratio.

==> correlation_tests.tex <==
\begin{table}
\centering
\begin{tabular}{lcccc}
\hline
Parameter & $\rho_{\rm p}$ & P$_{\rm p}$ & $\rho_{\rm s}$ & P$_{\rm s}$ \\ \hline \hline
M$_{\rm Ni}$               & 0.46       & 0.15       & 0.52        & 0.10         \\
M$_{\rm host}^{B}$         & -0.34      & 0.66       & 0.00        & 1.00           \\
M$_{\rm max}^{V}$          & -0.62      & 0.08       & -0.54       & 0.14        \\
s$_2$                      & 0.08       & 0.89       & -0.30       & 0.62        \\
OPT$_{\rm d}$              & -0.24      & 0.57       & -0.26       & 0.53        \\
vel(Fe II 5169)            & 0.30       & 0.40       & 0.13        & 0.73        \\
pEW(Fe II 5169)            & -0.43      & 0.47       & -0.70       & 0.19        \\
vel(Na I D)                & 0.44       & 0.46       & 0.50        & 0.39        \\
M$_{\rm prog}^{\rm K}$     & 0.62       & 0.10       & 0.59        & 0.13        \\
M$_{\rm prog}^{\rm SG}$    & 0.58       & 0.13       & 0.63        & 0.09        \\
E$_{\rm exp}$              & 0.45       & 0.44       & 0.30        & 0.62        \\
L$_{6300}$                 & 0.29       & 0.57       & 0.35        & 0.50         \\
L$_{6364}$                 & 0.18       & 0.74       & 0.35        & 0.50         \\
L$_{6300+6364}$            & 0.26       & 0.62       & 0.35        & 0.50         \\
L$_{6300}$/L$_{6364}$      & -0.20      & 0.70       & -0.35       & 0.50         \\
(12 + log(O/H))$_{\rm N2}$ & 0.01       & 0.99       & -0.60       & 0.40         \\ \hline
\end{tabular}
\caption{Pearson (subscript p) and Spearman (subscript s) correlation tests between the parameters listed and Ni/Fe ratio. $\rho$ are the correlation coefficients and P are the p-values. The velocities and pEW are measurements at 50 days after the explosion of each SN.}
\label{tab:correlation_tests}
\end{table}

==> sn_sample0.tex <==
\begin{table*}
\centering
\setlength\tabcolsep{3.5pt} % default value: 6pt
\begin{tabular}{lcccccccccc}
\hline
SN          & z        & M$_{\rm Ni}$& $\sigma_{\rm Ni}^-$ & $\sigma_{\rm Ni}^+$ & $\mu$& $\sigma_{\mu}$ & Host  & v$_{\rm vir}$& v$_{\rm 3k}$ & Ref. \\
  &        & [M$_{\odot}$] & [M$_{\odot}$]  & [M$_{\odot}$]  & [mag] &  &             & [km s$^{-1}$]& [km s$^{-1}$] \\ \hline\hline
SN1997D     & 0.004059 & 0.005                                                                & 0.004               & 0.004               & 30.74                                                 & 0.92           & NGC 1536        & 967                                                                   & 1261                                                                 & \citet{Spiro14}        \\
SN1999br    & 0.00323  & 0.002                                                                & 0.001               & 0.001               & 31.19                                                 & -              & NGC 4900        & 1041                                                                  & 1288                                                                 & \citet{Pastorello04}   \\
SN2002gd    & 0.00892  & <0.003                                                               & -                   & -                   & 32.87                                                 & 0.35           & NGC 7537        & 2702                                                                  & 2307                                                                 & \citet{Spiro14}        \\
SN2002gw     & 0.01028  & 0.012                                                                & 0.004               & 0.003               & 32.98                                                 & 0.23           & NGC 922        & 2872                                                                  & 2884                                                                 & \citet{Anderson14}     \\
SN2003B     & 0.00424  & 0.017                                                                & 0.009               & 0.006               & 31.11                                                 & 0.28           & NGC 1097        & 1028                                                                  & 1104                                                                 & \citet{Anderson14}     \\
SN2003fb    & 0.01754  & >0.017                                                               & -                   & -                   & 34.43                                                 & 0.12           & UGC 11522       & 5415                                                                  & 5012                                                                 & \citet{Anderson14}     \\
SN2003Z     & 0.0043   & 0.005                                                                & 0.003               & 0.003               & 31.70                                                 & 0.6            & NGC 2742        & 1483                                                                  & 1402                                                                 & \citet{Spiro14}        \\
SN2004fx    & 0.00892  & 0.014                                                                & 0.006               & 0.004               & 32.82                                                 & 0.24           & MCG -02-14-003  & 2474                                                                  & 2676                                                                 & \citet{Anderson14}     \\
SN2005cs    & 0.002    & 0.006                                                                & 0.003               & 0.003               & 29.46                                                 & 0.6            & M 51            & 718                                                                   & 634                                                                  & \citet{Spiro14}        \\
SN2007aa    & 0.004887    & 0.032                                                                & 0.009               & 0.009               & 31.95                                                 & 0.27            & NGC 4030            & 1483                                                                   & 1822                                                                  & This Work       \\
SN2008bk    & 0.000767 & 0.007                                                                & 0.0004              & 0.001               & 27.68                                                 & 0.05           & NGC 7793        & 59                                                                    & -52                                                                  & \citet{Anderson14}     \\
SN2008in    & 0.005224 & 0.015                                                                & 0.003               & 0.003               & 30.60                                                 & 0.2            & NGC 4303        & 1628                                                                  & 1912                                                                 & \citet{Roy11}          \\
SN2009N     & 0.003456 & 0.02                                                                 & 0.004               & 0.004               & 31.67                                                 & 0.11           & NGC 4487        & 1043                                                                  & 1384                                                                 & \citet{Takats14}       \\
SN2010id    & 0.01648  & -                                                                    & -                   & -                   & 32.86                                                 & 0.5            & NGC 7483        & 4964                                                                  & 4568                                                                 & \citet{Spiro14}        \\
SN2012A     & -  & 0.011                                                                 & 0.04               & 0.04               & 29.96                                                 & 0.15           & NGC 3239        & 798                                                                  & 1083         
                                          & \citet{Tomasella13}    \\
SN2012aw    & -  & 0.06                                                                 & 0.01               & 0.01               & 29.97                                                 & 0.03           & NGC 3351        & 810                                                                  & 1126          
                                          & \citet{Fraser12}    \\
SN2012ec    & 0.00469  & 0.04                                                                 & 0.015               & 0.015               & 31.19                                                 & 0.13           & NGC 1084        & 1268                                                                  & 1212                                                                 & \citet{Barbarino15}    \\
SN2013am    & 0.002692 & 0.015                                                                & 0.006               & 0.011               & 30.54                                                 & 0.4            & NGC 3623        & 863                                                                   & 1149                                                                 & \citet{Zhang14}        \\
%ASASSN-15oz & 0.006929 & 0.11                                                                 & 0.03                & 0.03                & 32.3                                                  & 0.2            & HIPASS J1919-33 & 2035                                                                  & 1940                                                                 & \citet{Bostroem19}     \\
SN2016aqf   & 0.004    & 0.011                                                                    & 0.001               & 0.001               & 30.51                                                 & 0.41            & NGC 2101        & 883                                                                   & 1262                                                                 & This Work              \\
SN2016bkv   & 0.002    & 0.0216                                                               & 0.0014              & 0.0014              & 30.79                                                 & 0.05           & NGC 3184        & 743                                                                   & 831                                                                  & \citet{Hosseinzadeh18} \\
%SN2016X     & 0.004408 & 0.032                                                                & 0.006               & 0.006               & 30.91                                                 & 0.43           & UGC 08041       & 1383                                                                  & 1652                                                                 & \citet{Huang18}        \\ \hline
\end{tabular}
\caption{SN II sample, with their respective host galaxies, used in this work. The redshift are as reported in the references cited in column Ref. (directly measured from spectra). The M$_{\rm Ni}$ and $\mu$ values (together with the uncertainties) were obtained from the references cited in column Ref.. The v$_{\rm vir}$ and v$_{\rm 3k}$ values were obtained from http://leda.univ-lyon1.fr/ (these could differ from the values used in the references as this website is updated when more accurate measurements are available or because they change the adopted cosmology [H$_0$]).}
\label{tab:sn_sample}
\end{table*}
